Stochastic triangular mesh mapping: A terrain mapping technique for autonomous mobile robots

For mobile robots to operate autonomously in general environments, perception is required in the form of a dense metric map. For this purpose, we present the stochastic triangular mesh (STM) mapping technique: a 2.5-D representation of the surface of the environment using a continuous mesh of triangular surface elements, where each surface element models the mean plane and roughness of the underlying surface. In contrast to existing mapping techniques, a STM map models the structure of the environment by ensuring a continuous model, while also being able to be incrementally updated with linear computational cost in the number of measurements. We reduce the effect of uncertainty in the robot pose (position and orientation) by using landmark-relative submaps. The uncertainty in the measurements and robot pose are accounted for by the use of Bayesian inference techniques during the map update. We demonstrate that a STM map can be used with sensors that generate point measurements, such as light detection and ranging (LiDAR) sensors and stereo cameras. We show that a STM map is a more accurate model than the only comparable online surface mapping technique$\unicode{x2014}$a standard elevation map$\unicode{x2014}$and we also provide qualitative results on practical datasets.

==> sections/equation_scratch.tex <==
\begin{equation}
  p(\mset{M}_s, \mset{Z}_s=\given{Z}_s | \mvec{\theta}_s)
  =
  \prod_i
  \phi_i(\mvec{\theta}_s, \mvec{m}_i, \mvec{z}_i).
\end{equation}

\begin{equation}
  \begin{split}
    \belief(\mset{\Theta})
    &\propto
    \int\displaylimits_{\mset{M}}
    p(\mset{\Theta}, \mset{M}, \mset{Z}=\given{Z})
    \, \text{d} \mset{M}\\
    &=
    \prod_{k}
    \phi_p(\mvec{\theta}_s)
    \int\displaylimits_{\mset{M}_s}
    p(\mset{M}_s, \mset{Z}_s=\given{Z}_s | \mvec{\theta}_s)
    \, \text{d}\mset{M}_s
  \end{split}
\end{equation}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% End:

==> sections/meas_model.tex <==
\section{Measurement Model}
\label{sec:measmodel}
There are several types of sensors used to observe spatial features in the
environment. Sensors such as lidar, radar, sonar, and depth-cameras, use active
time-of-flight to measure depth. Whereas a stereo-camera passively infers depth
from the measurements of two cameras. However, both these processes can be
modelled using a beam model, specifically: a measurement is said to originate
from a depth along the beam, whereby both the beam-width and depth are
uncertain. The main modelling concern is that of depth, which is dependent on
how the sensor operates. Therefore to simplify this we choose to model the
measurement process as the sampling of a point on a continuous surface, i.e. a
measurement is generated a single point. This model is applied irrespective of
the sensor type.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% End: 

==> sections/overview.tex <==
\section{Overview}
\label{sec:overview}

In the remainder of this paper we present and motivate the \acf{STM} mapping
technique, which addresses these key issues affecting dense mapping. First we
describe a method that addresses the issue of incorporating pose belief
uncertainty into the mapping process (\Cref{sec:irfs}), and then incorporating
statistical dependence between map elements using \iac{STM} map
(\Cref{sec:mapmodel}). We then present practical results of the \ac{STM} mapping
technique (\Cref{sec:results}), and conclude with a discussion and future work
(\Cref{sec:conclusion}).

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% End:

==> sections/rebuttal.tex <==
\section*{Response to Reviewers}

We would firstly like to thank both reviewers for their time, effort and
insightful comments, which has helped increase the quality of this manuscript.

\subsection*{Reviewer 1}

\begin{quote}
  The paper is very well written. The proposed method is sound and is validated
  by comprehensive results.

  Technically, the paper has provided a comprehensive discussion of existing
  work to set the ground of the proposed method. The proposed method is well
  presented with all technical details explained and justified.

  On the down side, the paper has provided an excessive amount of mathematical
  details, particularly under section 5.1. It could be improved to trim out part
  of the equations and focus the discussion only on more important parts. This
  can also help improve the readability of the paper and address the potential
  over-page problem of the paper.
\end{quote}

\paragraph{Authors' response}
This was also originally a concern of ours. We therefore chose to include only
the most relevant information---for example, we excluded the minimisation step
in \ac{VMP}, and only provided a very brief introduction to \acp{PGM}. We looked
also at slimming down the mathematical details in Section 5.1. This would save a
few pages, but to the detriment of a coherent derivation to our algorithm. The
algorithm should also be documented extensively for two main reasons. Firstly,
to our knowledge, this is the first time \ac{VMP} and \ac{LBP} has been
combined. Secondly, the \ac{VMP} algorithm requires the derivation of messages
for the specific problem it is being applied to. The algorithm presented is
therefore significantly different from existing algorithms, and not simply an
existing algorithm implemented for a specific application. We therefore could
not see how to significantly shorten the algorithm description without
introducing ambiguity, which would make the algorithm irreproducible. From the
review, it is also not clear which sections of the algorithm development are
obvious or unimportant and can be shortened without reducing the clarity of the
algorithm presentation. Additionally, as the current formatting of the paper is
for review purposes, if the paper were to be formatted to double column (in line
with the journal's formatting), the length of the article would decrease by
around 10 pages.


\subsection*{Reviewer 2}

\begin{quote}
  The paper proposes a stochastic triangular mesh mapping technique capable to
  model large terrain areas into a dense 3D metric map. The proposed technique
  employs a 2.5D representation of the surface using a continuous mesh of
  triangular surface elements, where each element models the local terrain mean
  plane and roughness. To reduce the effect of uncertainty in the robot pose,
  the authors consider landmark-relative submaps.

  According to the authors, the novel method is capable to incorporate
  uncertainty in the robot pose, incrementally update the map with reasonable
  computational complexity (O(N)), represent the statistical dependencies
  between map elements, and model the terrain surface explicitly.

  One positive aspect of the paper is the review and evaluation of possible
  approaches to deal with dense mapping. However, the current version of the
  paper is too long (41 pages); to facilitate the paper reading, the authors
  should consider resuming parts of the text.
\end{quote}

\paragraph{Authors' response}
Regarding the length of the paper, see the response to Reviewer 1.

\begin{quote}
  Also regarding the evaluation and comparison with other approaches, the
  authors mention that is unclear how the approximations made by the Hilbert
  maps framework will expand for less accurate sensors like stereo cameras. In
  this sense, the authors should also clarify the differences in the STM mapping
  results using accurate (laser) and inaccurate (camera) sensors.
\end{quote}

\paragraph{Authors' response}
The Hilbert maps framework is only demonstrated using LiDAR sensors, whereas we
demonstrate that STM mapping can successfully construct a map using measurements
from either a stereo camera or LiDAR sensor
(\Cref{sec:relative-irf-experiment,sec:global-irf-experiment}, respectively). In
contrast to Hilbert maps, we think that this alone is enough to show that STM
mapping works for both sensor modalities. This point is also not the focus of
the paper.

\begin{quote}
  The authors are representing the environment with a 2.5D map, which can not
  handle complex 3D shapes such as overhangs.
\end{quote}

\paragraph{Authors' response}
We are only limited to 2.5-D within each submap, and the combination of several
submaps could conceivably represent a fully 3-D environment. One could also
possibly use tetrahedron-shaped submaps, which would allow fully 3D maps. We
therefore think that the STM framework is extensible to allow for fully 3D maps.
However, we think that the 2.5-D formulation already constitutes a significant
contribution. We mention the possibilities for future work towards the end of
the paper (\Cref{sec:future-work}, line numbers \lineref{r1a}--\lineref{r1b}).

\begin{quote}
  Also, in lines 450--454 the authors comment that the associated surfel model
  does not try to exactly represent the actual surface of the terrain, but
  summarises the key aspects of the surface instead.
\end{quote}

\paragraph{Authors' response}
An STM map is an efficient representation for the purpose of robotic navigation,
since the model captures the relevant aspects of the environment, and avoids
modelling unnecessary details that are not relevant for the intended
application. We consider this to be an advantage rather than a disadvantage. To
clarify this point we have updated the text (\Cref{sec:surfel-model}, lines
\lineref{r7a}--\lineref{r7b}).

\begin{quote}
  Given the capability to deal with dense 3D metric maps of large areas, the STM
  mapping seems more suitable for autonomous terrestrial mobile robots
  navigating in large unknown terrains, instead of executing local tasks to
  obtain a precise model of objects with 3D complex geometry. This should be
  clarified in the text---also, the authors may consider changing the paper
  title to “Stochastic Triangular Mesh for Terrain Mapping”.
\end{quote}

\paragraph{Authors' response}
Thank you for raising a good point. Although we would like STM mapping to be
applicable to detailed object mapping, it is motivated by and tested only on
terrain mapping. Using a finer mesh would allow a more precise model, but this
currently unsubstantiated for the task of modelling complex 3-D objects. From
this suggestion we have renamed the article title to better clarify this point.
Our application to terrain mapping, however, does not limit STM mapping only to
terrestrial mobile robots, as a terrain map can also be applicable to aerial and
underwater robots. To make this point more explicit, wording has been added
(\Cref{sec:results}, line numbers \lineref{r2a}--\lineref{r2b}).

\begin{quote}
  The authors mention in lines 659--661 that the algorithms results differ
  noticeably with the exact believe when the measurement uncertainty is
  unreasonably high, but they did not encounter any issues when using simulation
  or practical data.
\end{quote}

\paragraph{Authors' response}
The current wording makes it seem like these points are contradictory. To
resolve this issue we clarified the wording of the paragraph
(\Cref{sec:infer-perf}, line numbers \lineref{r3a}--\lineref{r3b}).

\begin{quote}
  Also, the authors comment in lines 778--780 that convergence is not
  theoretically guaranteed, but they have not experienced any issues with
  convergence with their implementation. The paper does not present enough
  results to statistically validate such affirmations. These points should be
  further explored in the paper; also, a theoretical proof of convergence should
  be at least included as a future work to be investigated.
\end{quote}

\paragraph{Authors' response}
Thank you for raising another very valid point. Our algorithm is a combination
of both \ac{VMP} and \ac{LBP}, and although \ac{VMP} is guaranteed to converge,
\ac{LBP} on the other hand, does not have any convergence guarantees. Recent
work by \citet{Kamper2019} and \citet{Zhang2019} also shows that the convergence
of \ac{LBP} is still a topic of active research. Therefore, a formal proof would
probably not be possible. To clarify this point we have, however, expanded the
discussion into why we think our algorithm converges
(\Cref{sec:full-model-inference}, lines \lineref{r4a}--\lineref{r4b}). It should
also be noted that our algorithm was tested on both simulated and real data,
stereo camera and LiDAR sensor measurements, and in both relative and global
\acp{IRF}, and in all of these experiments our algorithm reliably converged
(despite this lack of a guaranteed convergence). Understandably though, future
work is required to provide a principled and in-depth analysis on the
convergence of our algorithm (\Cref{sec:future-work}, lines
\lineref{r5a}--\lineref{r5b}).

\begin{quote}
  The Relative Inertial Reference Frames methodology associates three landmarks
  to each submap. Also, the authors comment about considering the landmarks
  correlations to reduce the robot pose uncertainty. Such strategies are highly
  dependent on a robust and persistent identification of the landmarks, which is
  hard to guarantee during field operations. What about the STM mapping
  performance in such operation conditions?
\end{quote}

\paragraph{Authors' response}
We make the assumption that in order to use a relative \ac{IRF} the demarcating
landmarks need to be robustly and persistently identifiable. We then
demonstrated cases where this assumption is valid or unnecessary, namely:
\begin{itemize}
\item When artificial landmarks are place in the environment
  (\Cref{sec:relative-irf-experiment})
\item When accurate localisation is available from some other source
  (\Cref{sec:global-irf-experiment})
\end{itemize}
Although these cases do not yet allow the general operation we envision for
robotic vehicles, it demonstrates that our mapping technique is already
practically applicable. We also hope that this paper will stimulate research in
persistent identification of landmarks by highlighting its potential benefits.

\begin{quote}
  Figure 3 comments about a “practical stereo vision” dataset. The illustration
  in the graphical abstract does not represent a real robot---in fact, the paper
  makes no comments about any model of robotic device. The authors should
  present extra details about the data collection experiments and the robotic
  device employed in the tests.
\end{quote}

\paragraph{Authors' response}
Thank you for picking up on this. In \Cref{fig:corr_exp} we did not mention
anything about the data acquisition. To clarify this, we have updated the figure
caption to include a reference to the experiment that it was taken from. As
there was not motion in the dataset of this experiment (3 stationary stereo
image pairs), the practical setup focused only the sensors and not the full
robotic platform (\Cref{sec:relative-irf-experiment}, lines
\lineref{r6a}--\lineref{r6b}). Although we could discuss the full robotic
platform setup, this would provide unnecessary information.

\subsection*{Other Changes}
\begin{itemize}
\item Some of the figure sizes have been increased for readability.
\item Minor grammar changes have been incorporated.
\item Added a link to our source code.
\end{itemize}

\nolinenumbers
\bibliographystyle{elsarticle-num-names} % This can't use back-ref
% \bibliographystyle{IEEEtranN} % This works with back ref
\bibliography{bib/rebut_ref}
\linenumbers

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% End:
